Generation-Heavy Hybrid Machine Translation

The state of the art techniques in Machine Translation (MT) require large amounts of symmetric resources from source and target languages. This is true regardless of whether the approach is Transfer or Interlingua, Symbolic or Statistical. Symmetry within these approaches is necessary to ensure quality, robustness and retargetability. In reality, such symmetry, whether it is in terms of structural transfer lexicons, interlingual dictionaries or parallel corpora, is a major bottleneck in developing any MT system. This dissertation presents an approach to MT that addresses the lack of symmetry by exploiting symbolic and statistical target language resources in source-poor/target-rich language pairs. This approach is called Generation-Heavy Hybrid Machine Translation (GHMT). Expected source language resources include a syntactic parser and a simple one-to-many translation dictionary. No transfer rules or complex interlingual representations are used. Rich target language symbolic resources are used to overgenerate multiple structural variations from a target-glossed syntactic dependency representation of source language sentences. Statistical target-language resource are then used to select amongst the overgenerated translations. The source-target asymmetry of systems developed in this approach makes them more easily retargetable to new source languages.

==> graphics/sen23-rest <==
#FIG 3.2
Landscape
Center
Inches
Letter  
100.00
Single
-2
1200 2
6 898 2700 1798 2925
2 4 0 1 0 7 50 0 -1 0.000 0 0 7 0 0 5
	 1798 2925 1798 2700 898 2700 898 2925 1798 2925
4 0 0 50 0 16 12 0.0000 4 180 420 1135 2875 *pro*\001
-6
6 3008 2700 4958 4185
6 4058 3450 4958 4185
2 4 0 1 0 7 50 0 -1 0.000 0 0 7 0 0 5
	 4958 4185 4958 3450 4058 3450 4058 4185 4958 4185
4 0 0 50 0 16 12 0.0000 4 135 645 4215 3615 ultimate\001
4 0 0 50 0 16 12 0.0000 4 135 750 4145 4125 hindmost\001
4 0 0 50 0 16 12 0.0000 4 135 345 4345 3785 final\001
4 0 0 50 0 16 12 0.0000 4 135 285 4385 3965 last\001
-6
6 3008 3440 3908 3665
2 4 0 1 0 7 50 0 -1 0.000 0 0 7 0 0 5
	 3908 3665 3908 3440 3008 3440 3008 3665 3908 3665
4 0 0 50 0 16 12 0.0000 4 135 285 3305 3610 this\001
-6
6 3588 2700 4488 2925
2 4 0 1 0 7 50 0 -1 0.000 0 0 7 0 0 5
	 4488 2925 4488 2700 3588 2700 3588 2925 4488 2925
4 0 0 50 0 16 12 0.0000 4 135 570 3770 2865 missile\001
-6
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 3
	 3448 3440 4018 2930 4508 3460
-6
6 1948 2700 2848 3435
2 4 0 1 0 7 50 0 -1 0.000 0 0 7 0 0 5
	 2848 3435 2848 2700 1948 2700 1948 3435 2848 3435
4 0 0 50 0 16 12 0.0000 4 135 450 2185 3020 could\001
4 0 0 50 0 16 12 0.0000 4 180 450 2185 3360 might\001
4 0 0 50 0 16 12 0.0000 4 135 345 2235 3170 may\001
4 0 0 50 0 16 12 0.0000 4 90 300 2245 2850 can\001
-6
6 3728 1350 4628 2085
2 4 0 1 0 7 50 0 -1 0.000 0 0 7 0 0 5
	 4628 2085 4628 1350 3728 1350 3728 2085 4628 2085
4 0 0 50 0 16 12 0.0000 4 180 465 3935 1490 equip\001
4 0 0 50 0 16 12 0.0000 4 120 705 3845 2010 accouter\001
4 0 0 50 0 16 12 0.0000 4 90 390 3975 1840 crew\001
4 0 0 50 0 16 12 0.0000 4 135 555 3905 1680 furnish\001
-6
6 5708 1360 6608 1585
2 4 0 1 0 7 50 0 -1 0.000 0 0 7 0 0 5
	 6608 1585 6608 1360 5708 1360 5708 1585 6608 1585
4 0 0 50 0 16 32 0.0000 4 45 135 6083 1500 .\001
-6
6 4788 595 5688 840
2 4 0 1 0 7 50 0 -1 0.000 0 0 7 0 0 5
	 5688 840 5688 615 4788 615 4788 840 5688 840
4 0 0 50 0 16 12 0.0000 4 135 465 5005 790 *root*\001
-6
6 5166 3465 6066 3690
2 4 0 1 0 7 50 0 -1 0.000 0 0 7 0 0 5
	 6066 3690 6066 3465 5166 3465 5166 3690 6066 3690
4 0 0 50 0 16 12 0.0000 4 135 615 5316 3630 nuclear\001
-6
6 5776 2700 6676 2925
2 4 0 1 0 7 50 0 -1 0.000 0 0 7 0 0 5
	 6676 2925 6676 2700 5776 2700 5776 2925 6676 2925
4 0 0 50 0 16 12 0.0000 4 135 720 5876 2870 warhead\001
-6
6 6436 5405 7336 5780
2 4 0 1 0 7 50 0 -1 0.000 0 0 7 0 0 5
	 7336 5780 7336 5405 6436 5405 6436 5780 7336 5780
4 0 0 50 0 16 12 0.0000 4 135 480 6688 5725 which\001
4 0 0 50 0 16 12 0.0000 4 135 300 6738 5555 that\001
-6
6 5386 5405 6286 5630
2 4 0 1 0 7 50 0 -1 0.000 0 0 7 0 0 5
	 6286 5630 6286 5405 5386 5405 5386 5630 6286 5630
4 0 0 50 0 16 12 0.0000 4 180 420 5623 5580 *pro*\001
-6
6 6426 3455 7326 4925
2 4 0 1 0 7 50 0 -1 0.000 0 0 7 0 0 5
	 7326 4925 7326 3455 6426 3455 6426 4925 7326 4925
4 0 0 50 0 16 12 0.0000 4 120 510 6618 3605 create\001
4 0 0 50 0 16 12 0.0000 4 135 375 6708 4840 bear\001
4 0 0 50 0 16 12 0.0000 4 135 465 6638 4670 afford\001
4 0 0 50 0 16 12 0.0000 4 135 630 6578 4490 activate\001
4 0 0 50 0 16 12 0.0000 4 180 390 6678 4325 yield\001
4 0 0 50 0 16 12 0.0000 4 180 675 6578 4145 produce\001
4 0 0 50 0 16 12 0.0000 4 135 450 6638 3965 make\001
4 0 0 50 0 16 12 0.0000 4 90 495 6628 3785 cause\001
-6
6 7410 5400 8310 5625
2 4 0 1 0 7 50 0 -1 0.000 0 0 7 0 0 5
	 8310 5625 8310 5400 7410 5400 7410 5625 8310 5625
4 0 0 50 0 16 12 0.0000 4 135 450 7650 5570 israel\001
-6
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1348 2680 4198 2080
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2408 2700 4168 2090
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4048 2680 4148 2090
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4168 2080 6198 2690
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5228 850 4128 1350
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5218 850 6168 1360
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 3
	 5616 3465 6226 2915 6836 3445
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 3
	 5836 5405 6876 4915 6876 5405
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6886 4935 7926 5395
4 0 0 50 0 14 12 0.0000 4 180 1365 5415 2430 at,by,with...\001
4 0 0 50 0 14 12 0.0000 4 150 1680 7500 5175 about,within,...\001
4 0 0 50 0 14 12 0.0000 4 180 525 5685 5175 :subj\001
4 0 0 50 0 14 12 0.0000 4 180 420 6900 5295 :obj\001
4 0 0 50 0 14 12 0.0000 4 135 525 3915 1140 :main\001
4 0 0 50 0 14 12 0.0000 4 135 210 5805 1125 :*\001
4 0 0 50 0 14 12 0.0000 4 135 420 6615 3210 :mod\001
4 0 0 50 0 14 12 0.0000 4 135 420 5385 3255 :mod\001
4 0 0 50 0 14 12 0.0000 4 180 525 1635 2505 :subj\001
4 0 0 50 0 14 12 0.0000 4 180 420 4095 2565 :obj\001
4 0 0 50 0 14 12 0.0000 4 135 420 2910 2640 :mod\001
4 0 0 50 0 14 12 0.0000 4 135 420 4350 3300 :mod\001
4 0 0 50 0 14 12 0.0000 4 135 420 3180 3270 :mod\001

